GrACE: Generation using Associated Code Edits

Developers expend a significant amount of time in editing code for a variety of reasons such as bug fixing or adding new features. Designing effective methods to predict code edits has been an active yet challenging area of research due to the diversity of code edits and the difficulty of capturing the developer intent. In this work, we address these challenges by endowing pre-trained large language models (LLMs) of code with the knowledge of prior, relevant edits. The generative capability of the LLMs helps address the diversity in code changes and conditioning code generation on prior edits helps capture the latent developer intent. We evaluate two well-known LLMs, Codex and CodeT5, in zero-shot and fine-tuning settings respectively. In our experiments with two datasets, the knowledge of prior edits boosts the performance of the LLMs significantly and enables them to generate 29% and 54% more correctly edited code in top-1 suggestions relative to the current state-of-the-art symbolic and neural approaches, respectively.

==> help/todos.tex <==
\section{TODO and Help}

\subsection*{TODOs}
To write the todos mention the name to who the todo is assigned. See the Help guide for the maros.
\begin{enumerate}
    \item \ashish{Should we include Edit Similarity? We have good Exact Match numbers and the edit similarity metric can be misleading at times.}
\end{enumerate}

\subsection*{Help}
\begin{itemize}
    \item To write full code (mind the spacing of the code in the latex file),
\lstset{escapechar=@,style=CustomCS}
\begin{lstlisting}
    protected virtual void AppendMethod(
        StringBuilder sb, Exception ex){
        // A line comment on the code
        sb.Append("Hello World!");
#if SILVERLIGHT | | NETSTANDARD1_0
        sb.Append(
            ParseMethodNameFromStackTrace(
                ex.StackTrace
            )
        );
#endif
        /* 
        * Finally a block comment
        */
    }
\end{lstlisting} 
    \item To write a code in one line, \linecode{public static void main (String args[])}
    \item To highlight something with a box, \\\highlight{This line needs to be highlighted}
    \item For writing any code with error \errorcode{statioc void main}
    \item To highlight a lesson learned, \lessons{lesson learned}
    \item To \textbf{start} a research question  \RQ{The question} Note that, when you start a new RQ, the number will be automatically updated. 
    \item To \textbf{repeat} an earlier research question \RQrepeat{1}{The question}
    \item To \textbf{answer} a RQ \RS{1}{The answer}.
    \item To leave comment for specific persons,
        \begin{itemize}
            \item \ashish{For assigning to Ashish}
            \item \aditya{For assigning to Aditya}
            \item \priyanshu{For assigning to Priyanshu}
            \item \avishree{For assigning to Avishree}
            \item \gustavo{For assigning to Gustavo}
            \item \arjun{For assigning to Arjun}
            \item \saikat{For assigning to Saikat}
            \item \yasharth{For assigning to Yasharth}
            \item \todo{\red{\emph{Please add macros for others' names as necessary in the \underline{\tt includes/macros.tex}.}}}
            
        \end{itemize}
\end{itemize}
